Infection Pressure on Fish in Cages

We address the question of how to connect predictions by hydrodynamic models of how sea lice move in water to observable measures that count the number of lice on each fish in a cage in the water. This question is important for management and regulation of aquacultural practice that tries to maximise food production and minimise risk to the environment. We do this through a simple rule-based model of interaction between sea lice and caged fish. The model is simple: sea lice can attach and detach from a fish. The model has a novel feature, encoding what is known as a master equation producing a time-series of distributions of lice on fish that one might expect to find if a cage full of fish were placed at any given location. To demonstrate how this works, and to arrive at a rough estimate of the interaction rates, we fit a simplified version of the model with three free parameters to publicly available data about an experiment with sentinel cages in Loch Linnhe in Scotland. Our construction, coupled to the hydrodynamic models driven by surveillance data from industrial farms, quantifies the environmental impact as: what would the infection burden look like in a notional cage at any location and how does it change with time?

==> Makefile <==
all: cagedata cagehist simulated fit plots paper kappa

cagedata: .cagedata
.cagedata: data/Sentinel_cage_sampling_info_update_01122022.csv
	python ./src/pertsplit.py $< data/linnhe
	touch .cagedata

cagehist: .cagehist
.cagehist:
	for cage in data/linnhe/cage_*.tsv; do \
		htsv="`echo $$cage | sed -e s/linnhe/histograms/ -e s/cage/hist/`"; \
		python ./src/linnhe.py $$cage count > $$htsv; \
	done
	touch .cagehist

simulated: data/simulated/density-timeseries.tsv density-sweep beta-sweep gamma-sweep

data/simulated/density-timeseries.tsv:
	python ./src/cmsim.py -l 360 -i 24 -c 0 --dimensions 20 > data/simulated/density-timeseries.tsv

density-alone: data/simulated/density-sweep-b0.02-g0.01-d${dens}.tsv
data/simulated/density-sweep-b0.02-g0.01-d${dens}.tsv:
	python ./src/cmsim.py --dimensions 20 -l 360 --density ${dens} > $@
density-sweep:
	for dens in 0.01 0.1 1.0 10.0; do make dens=$$dens density-alone; done

beta-alone: data/simulated/beta-sweep-b${beta}-g0.01-d0.1.tsv
data/simulated/beta-sweep-b${beta}-g0.01-d0.1.tsv:
	python ./src/cmsim.py --dimensions 20 -l 360 --beta0 ${beta} --beta1 ${beta} > $@
beta-sweep:
	for beta in 0.01 0.02 0.03 0.04 0.05; do make beta=$$beta beta-alone; done

gamma-alone: data/simulated/gamma-sweep-b0.02-g${gamma}-d0.1.tsv
data/simulated/gamma-sweep-b0.02-g${gamma}-d0.1.tsv:
	python ./src/cmsim.py --dimensions 20 -l 360 --gamma ${gamma} > $@
gamma-sweep:
	for gamma in 0.0 0.005 0.01 0.015 0.02; do make gamma=$$gamma gamma-alone; done

fit: data/fitting/fitting-summary.tsv
	make season=spring fitting-season-split
	make season=autumn fitting-season-split
data/fitting/fitting-summary.tsv:
	echo 'filename\tcolumn\tcage\tyyyy\tseason\tnfish\tduration\tdensity\tbeta0\tbeta1\tgamma\tdist' > $@
	for dat in data/linnhe/*.tsv; do \
		python ./src/cmfit.py $$dat duration count >> $@.$$; \
	done
	< $@.$$ sort -k6 -n >> $@
	rm -f $@.$$
fitting-season-split: data/fitting/fitting-summary-${season}.tsv
data/fitting/fitting-summary-${season}.tsv: data/fitting/fitting-summary.tsv
	head -1 $< > $@
	grep ${season} $< | sort -k6 -n >> $@

plots: data/fitting/fitting-summary.tsv
	python ./src/aplot.py data/fitting/fitting-summary.tsv data/simulated

paper: copepod-master.pdf
copepod-master.pdf: copepod-master.aux copepod-master.bbl
	pdflatex -interaction=nonstopmode copepod-master
	pdflatex -interaction=batchmode copepod-master
copepod-master.bbl: copepod-master.aux refs.bib
	bibtex copepod-master
copepod-master.aux: copepod-master.tex refs.bib
	pdflatex -interaction=nonstopmode copepod-master

kappa: src/cm.ka
src/cm.ka: src/cm.ska
	python ./src/stratify.py $< $@ -fix beta0=0.0175 beta1=0.0225 gamma=0.005

clean:
	rm -f data/linnhe/*
	rm -f data/histograms/*
	rm -f data/simulated/*
	rm -f data/fitting/*
	rm -f *.aux *.bbl *.blg *.log
	rm -f src/cm.ka
	rm -f .cagedata .cagehist

